On Learning Representations for Tabular Data Distillation

Dataset distillation generates a small set of information-rich instances from a large dataset, resulting in reduced storage requirements, privacy or copyright risks, and computational costs for downstream modeling, though much of the research has focused on the image data modality. We study tabular data distillation, which brings in novel challenges such as the inherent feature heterogeneity and the common use of non-differentiable learning models (such as decision tree ensembles and nearest-neighbor predictors). To mitigate these challenges, we present $\texttt{TDColER}$, a tabular data distillation framework via column embeddings-based representation learning. To evaluate this framework, we also present a tabular data distillation benchmark, ${{\sf \small TDBench}}$. Based on an elaborate evaluation on ${{\sf \small TDBench}}$, resulting in 226,890 distilled datasets and 548,880 models trained on them, we demonstrate that $\texttt{TDColER}$ is able to boost the distilled data quality of off-the-shelf distillation schemes by 0.5-143% across 7 different tabular learning models.

==> pipeline_desc.tex <==
\section{Tabular Data Distillation Benchmark}

\subsection{Tabular Data Distillation Pipeline}
\label{sec:pipeline_desc}
%
Data distillation has been mostly studied in the context of images where each data point is composed of a homogeneous set of features - pixels - and the downstream models are neural networks.
The two main distinctions with tabular data distillation are: (i)~\textbf{Feature Heterogenity}: Features in tabular data are usually heterogeneous and can have vastly different meanings, making it challenging to generate appropriate feature aggregations as usually done with neural networks.
This is further exacerbated by the common presence of missing values.
(ii)~\textbf{Model Variety}: The types of downstream models can vary significantly, although the most successful models are often tree-based~\cite{grinsztajnWhyTreebasedModels2022,shwartz-zivTabularDataDeep2022}.
However, neural networks ~\cite{gorishniyRevisitingDeepLearning2021,guoDeepFMFactorizationMachineBased2017} as well as linear and nearest-neighbor models are also commonly used (e.g., for interpretability reasons).

While developing a tabular data distillation pipeline, we make a deliberate attempt to address these points.
We consider a classification dataset $S = \{(x_1, y_1), \ldots, (x_N, y_N)\}$ with $N$ examples, $r$ numerical features and $c$ categorical features (i.e. $x_i \in \mathbb R^r \times \mathbb C^c$) and $L$ labels (that is, $y_i \in Y = \{1, \ldots, L\}$).
We allow the features to contain missing values.
We propose the following steps for tabular data distillation:
%
\begin{itemize}
 	\item Data homogenizing: An encoder $P: \mathbb R^r \times \mathbb C^c \to \{0, 1\}^D$ that maps the heterogeneous tabular features to a (superficially) homogeneous very high dimensional (but very) sparse Hamming space.
	\item Encoding in latent space: An encoder $\phi: \{0, 1\}^D \to \mathbb R^d, d \ll D$ that maps the high dimensional sparse binary features to a rich dense low-dimensional space.
	\item Decoding latent representation: A decoder $\psi: \mathbb R^d \to \mathbb R^D$, that decodes the latent representation generated by $\phi$ back to the high dimensional space.
	\item (Optional) Supervised latent space fine-tuning: A classifier $f: \mathbb R^d \to Y$ that utilizes the latent representations for predicting the class.
	\item Distilling data in latent space: A data distiller $F: \mathbb R^{N \times d} \to \mathbb R^{n \times d}, n \ll N$ which distills the $N$ samples in the latent space to $n$ samples.
\end{itemize}
%
The goal of the data homogenizing is to convert mixed numerical and categorical with missing values into a homogeneous representation to mitigate the effect of the inherent heterogeneity between the features in tabular data.
Converting the data into a binary representation across all feature types enables us to leverage modern NN-based representation learning schemes.
However, this sparse high dimensional homogeneous representation is not necessarily conducive to data distillation.
For example, Euclidean clustering is a strong distillation baseline~\cite{cuiDCBENCHDatasetCondensation2022}, but clustering is known to be a computationally hard problem in sparse and high dimensional data~\cite{assentClusteringHighDimensional2012,steinbachChallengesClusteringHigh2004}.

Thus, we utilize an encoder $\phi: \{0,1\}^D \to \mathbb R^d$ to map samples in the sparse high dimensional space to a low-dimensional dense representation, where clustering and other data compression schemes are relatively easier.
The decoder $\psi:\mathbb R^d \to \mathbb R^D$ allows us to learn high-fidelity dense low-dimensional representations that minimize the information loss between the high-dimensional binary representations and the low-dimensional dense representations.
This is achieved by training an autoencoder using $\phi$ (encoder) and $\psi$ (decoder).
The encoder-decoder pair also allows us to perform data distillation in a downstream model agnostic manner.

However, learning the encoder solely by minimizing the autoencoder reconstruction loss implies that the low-dimensional latent space representations do not incorporate any information regarding the labels of the samples and solely rely on the features.
Since the goal is to achieve high predictive performance with the downstream model trained on the distilled data, we also consider an additional optional step of supervised fine-tuning of the latent space representations with a classifier head that predicts the sample labels utilizing their latent space representations.
This fine-tuning phase is employed after the autoencoder is fully trained, ensuring that the reconstruction loss remains low.

\vspace{-8px}
\paragraph{Application-dependent downstream processing.}
Given the distilled data $\bar S$ with $n$ samples in the latent space, we consider the following forms of downstream use for model training:
%
% \begin{itemize}
% \item We form a new distilled set $\widetilde S$ of $n$ samples such that all the $n$ samples correspond to original examples in $S$. For this, we find the closest point in $S$ in the same class for each sample in $\bar S$ in the latent space. That is $\widetilde S = \{ \arg \min_{(x, y) \in S, y = y'} \|z - \phi(P(x))\|_2, \forall (z, y') \in \bar S \}$. 
% \item We use the distilled data $\widetilde S_{e}$ \todo{Is $\widetilde S_{e}$ the same as $\bar S$? }in the latent space to train the downstream model. It is important to note that this choice will require us to have the data homogenizer $P$ and the encoder $\phi$ for inference with the downstream model.
% \item We decode the distilled data $n$ samples in $\widetilde S_{e}$ using the decoder $\psi$ to get $\widetilde S_{d} = \{(\sigma(\psi(z)), y), \forall (z,y) \in \widetilde S_{e}\}$, where $\sigma: \mathbb R^D \to [0,1]^D$ is a group-wise softmax operator.\footnote{We will describe this in detail.} We then use the $\hat S$ \todo{is $\hat S$ the same as $\widetilde S_{d}$?} to train the downstream model. In this case, we do not require to have the encoder $\phi$ for inference with the downstream model though we still need the data homogenizer $P$. 
% \end{itemize}
% %
% These different options can not only be performance driven, but also application driven. For example, in some applications, it is more meaningful to have the distilled data be actual data samples as in $\widetilde S$, while in other applications, it is more beneficial to utilize artificial samples as in $\widetilde S_{e}$ or $\widetilde S_{d}$ to avoid sharing actual data for privacy concerns. Thus, it might be beneficial for downstream modeling to utilize the distilled data $\widetilde S_{e}$ in the latent space, but in some application, it might be necessary to consider the decoded version $\widetilde S_d$ to have interpretable features in the distilled data. If we train an interpretable downstream model (such as a linear model or a decision tree), then the decoded distilled data would allow us to generate global and local interpretations in terms of the more meaningful original features.
%

\begin{itemize}
	% \item We form a new distilled set $\widetilde S$ of $n$ samples such that all the $n$ samples correspond to original examples in $S$. For this, we find the closest point in $S$ in the same class for each sample in $\bar S$ in the latent space. That is $\widetilde S = \{ \arg \min_{(x, y) \in S, y = y'} \|z - \phi(P(x))\|_2 \forall (z, y') \in \bar S \}$. 
	\item We use the distilled data $\bar S$ in the latent space to train the downstream model. It is important to note that this choice will require us to have the data homogenizer $P$ and the encoder $\phi$ for inference with the downstream model.
	\item We decode the distilled data $n$ samples in $\bar S$ using the decoder $\psi$ to get $\hat S = \{(\sigma(\psi(z)), y) \forall (z,y) \in \bar S\}$, where $\sigma: \mathbb R^D \to [0,1]^D$ is a group-wise softmax operator. This choice does not require encoder $\phi$ for inference, though the data homogenizer $P$ is still needed.
 % \footnote{We will describe this in detail.} 
 % We then use the $\hat S$ to train the downstream model. In this case, we do n.
\end{itemize}
%
These different options can be performance driven or application driven.
% For example, in some applications, it is more meaningful to have the distilled data be actual data samples as in $\widetilde S$, while in other applications, it is more beneficial to utilize artificial samples as in $\bar S$ or $\hat S$ to avoid sharing actual data for privacy concerns.
% For example, in some applications, it is more meaningful to have the distilled data be in the same space as the actual data as in $\hat S$ for interpretability purposes, while in other applications, it is more beneficial to utilize a dense latent space $\bar S$ to avoid sharing the actual features for privacy concerns.
While it might be beneficial for the downstream model to utilize the distilled data $\bar S$ in the latent space, in some other applications, it might be necessary to consider the decoded version $\hat S$ to have interpretable features in the distilled data. If we train an interpretable downstream model (such as a linear model or a decision tree), then the decoded distilled data would allow us to generate global and local interpretations in terms of the more meaningful original features.

\subsubsection{Data homogenizing} \label{sec:pipeline_desc:dh}
%
\todo[inline]{
Instead, consider a ``Column Embedding'' section:
Given the input data, with appropriate conversion to a numerical form, we can directly apply a distillation scheme (such as clustering or gradient matching). Alternately, we can make use of column embeddings for tabular data. Column embeddings allow us to use encoders for representation learning based on modern architectures such as transformers and graph neural networks. With column embeddings, each of the $D$ columns in a table row is represented with a vector (say in $\R^d$, instead of a scalar), representing a row with $D$ vectors in $\R^d$. This $\R^{D \times d}$ representation of a row is then processed downstream.
While column embeddings are standard for categorical columns -- each category is represented with a vector, there are various ways of embedding numerical columns such as binning (the numerical features is binned, with each bin treated as a category), linear scaling (each value $v \in \R$ is converted to an embedding by multiplying it a shared vector $\mathbf{e} \in \R^d$ to get $v \mathbf{e}$), and PLE~\citep{gorishniyEmbeddingsNumericalFeatures2022}.
In the main text, we focus on the binned numerical features for a couple of reasons: (i)~The binned features naturally handle missing values (quite prevalent in tabular data) instead of relying on a heuristic intermediate imputation step (sometimes, the fact that a value is missing is in itself a signal, and heuristic imputation schemes often lose this information), and (ii)~The binned features can be used for all architectures we consider here -- feed-forward, graph neural-networks, and transformers -- and using a common embedding scheme allows us to ablate the effect of the different architectures. The other numerical embedding schemes do not apply to graph neural networks.
In the appendix, focusing on the transformers, we discuss the difference between the different numerical embedding schemes.
}
\todo{
Position this as an option we tried to use GNN and Trf; other option we tried was to distill in original-mixed space;
we could have tried original-mixed+FFN-enc+Distill but I dont think we have that
}
Given a dataset with $r$ numerical features and $c$ categorical features, we convert it to a sparse binary representation as follows: A categorical feature $i_c \in \{1, \ldots, c\}$ with $m_{i_c}$ categories is converted into a $m_{i_c}$-dimensional binary representation via one-hot encoding.
A numerical feature $i_r \in \{1, \ldots, r\}$ is binned into a pre-specified number of bins $m_{i_r}$, and then converted into a $m_{i_r}$-dimensional one-hot encoding treating the bin indices as categories.
In the presence of missing values, we can allocate an additional ``missing'' category for each of the categorical features, and an additional bin for missing values for each of the numerical features.
Finally, all the per-feature binary representations are concatenated to obtain a $D$-dimensional binary vector where $D = \sum_{i_c = 1}^c m_{i_c} + \sum_{i_r = 1}^r m_{i_r}$.
This representation is extremely sparse, with only $(c+r)$ nonzeros out of $D$ dimensions for each sample.

We would like to highlight a few aspects of this process: First, this scheme allows us to natively handle missing values, which are common in tabular data, without any additional step of missing value imputation.
The subsequent latent space encoding implicitly handles the missing values in an input-dependent manner without requiring explicit imputation.
Second, the binning of the numerical features might appear to be lossy, but is quite common~\cite{chenXGBoostScalableTree2016a,gorishniyEmbeddingsNumericalFeatures2022,keLightGBMHighlyEfficient2017,wangTransTabLearningTransferable2022}.
This binning or discretization of numerical tabular features has been used in the implementations of popular tree-based packages such as XGBoost and LightGBM for the purposes of efficiency without any loss in predictive performance or even gains.
Various recent neural networks for tabular data~\cite{gorishniyEmbeddingsNumericalFeatures2022,wangTransTabLearningTransferable2022} have also utilized such discretization.
Our distillation pipelines using this binning scheme are compared against a baseline that does not use any binning, validating this approach.
%\todo{cite FM transformer and PLE paper} 
%
\subsubsection{Encoding \& Decoding in latent space} \label{sec:pipeline_desc:ae}
% \todo{instead of MLP vs GNN, can we have labels of FFN vs GNN?}
%
To generate dense low dimensional representations $z \in \mathbb R^d$ from the sparse binary representations $b \in \{0, 1\}^D$, we start with a column embedding~\cite{chengWideDeepLearning2016} which maintains a weight vector $w_i \in \mathbb R^M$ for each $i \in \{1, \ldots, D\}$. We implement three distinct architectures for the encoder head to ablate the effectiveness of each architecture when representing tabular data -- \textit{fully-connected feed-forward network}, \textit{graph neural network} and \textit{transformer}.
We consider two training modes for each architecture: unsupervised training and supervised-fine-tuning (SFT). 
The goal of SFT is to embed the label information addition to the features in the latent space.
To preserve the reconstruction accuracy of the autoencoders, we attach a classifier head to the fully-trained (unsupervised) autoencoder and fine-tune on a combined loss function balanced by $\alpha$.
We treat $\alpha$ as a hyperparamter and tune the value for each dataset in our HPO step.
\Cref{apdx:sec:ae_imp_detail} discusses the implementation details of each architecture.
We consider the distilled data in both latent space and the decoded (reconstructed) space.
When the distillation algorithm is clustering-based and is using the median points (point closest to the Euclidean center) instead of the centroid, we also consider an additional case where we use the original version of the median point instead of the latent or decoded version.
% \todo{this line might need some fixing -- for example, what ``can be pointed back'' and what do we mean by ``point back''.  }
% \todo{I do not see the supervised fine-tuning or SFT step description anywhere around here. What am i missing?}
%
%
\subsubsection{Data distillation} \label{sec:pipeline_desc:dd}
%
A data distillation scheme takes as input a set of $N$ samples, and outputs a smaller set with $n \ll N$ samples.
We consider random sample as our baseline, which has also shown strong performance in image distillation~\cite{cuiDCBENCHDatasetCondensation2022}.
We discuss the 4 types of distillation methods we consider in this work below. 
Further details about the parameters used for each method can be found in~\cref{apdx:subsec:dd_params}. 
% Many of these schemes depend on the downstream neural network models.
% With tabular data, the downstream model can be anything from tree-based ensembles to nearest-neighbor ones.
% For this reason, we consider distillation schemes that are agnostic to the downstream model: two clustering-based scheme and kernel-machine based kernel-inducing points or KIP scheme~\cite{nguyen_dataset_2021}.

%\paragraph{Clustering-based distillation}
% We consider two types of clustering -- $k$-means clustering and hierarchical agglomerative clustering.
% Our goal is to test whether a distance-based or hierarchical clustering approach is more effective for distilling tabular data.
% While clustering is a straightforward method,~\citet{cuiDCBENCHDatasetCondensation2022} highlighted that it is a very strong baseline.
% Given $L$ classes, and $n$ desired distilled samples, we perform per-class clustering of the samples (in the latent space) with $n/L$ clusters per class, and use the per-cluster representatives (with their corresponding classes) to get a total of $n$ labeled samples.
% \todo{write this out mathematically?}

% \begin{wrapfigure}{l}{.4\textwidth}
%   \centering
%   \includegraphics[width=.4\textwidth]{figures/data_distill_desc.pdf}
%   \caption{Visual example of clustering-based distillation}
%   \label{fig:clsuter_distill_example}
% \end{wrapfigure}

{\bf $K$-means} finds $N/l$ clusters for each $l$ label group to produce a distilled dataset with $N$ points.
We consider multiple variations of this method -- by using the euclidean center of each cluster or the closest \textit{real} point to the euclidean center of each cluster.

{\bf Agglomerative} is similar to $k$-means, but the clustering algorithm is replaced by agglomerative clustering~\cite{mullnerModernHierarchicalAgglomerative2011}.
Specifically, we use the algorithm implemented by scikit-learn~\cite{scikit-learn} with `ward' linkage and `euclidean' distance metric.
Similarly to $k$-means, we also consider the \textit{real} and the \textit{synthetic} points of each cluster by computing the euclidean center of each cluster.

{\bf Gradient Matching (GM)~\cite{zhaoDatasetGradientMatching2021}} produces the distilled dataset by \textit{learning} a set of weights that induce similar gradients on a target model as if it were being trained on the original dataset. 
More formally, the optimization function for learning the distilled dataset can be written as follows:
%
\begin{equation}
    \min_{S}E_{\theta_0 \sim P_{\theta_0}}[\textstyle{\sum_{t=0}^{T-1}}D(\nabla_\theta \mathcal{L}^\mathcal{S}(\theta_t), \nabla_\theta \mathcal{L}^{\mathcal{T}}(\theta_t)) ]
\label{eq:dc_loss}
\end{equation}
%
where $T$ is the number of training iterations and $\mathcal{T}$ and $\mathcal{S}$ denote the original (target) and distilled (synthetic) datasets, respectively.

{\bf KIP~\cite{nguyenDatasetMetaLearningKernel2021}} uses neural tangent kernel (NTK) of a wide neural network produce a distill dataset.
Given a pair of feature matrix $X \in \mathbb R^{N \times d}$ and label vector $\mathbf y \in Y^N$, KIP learns a pair of feature matrix $X_s \in \mathbb R^{n \times d}$ and label vector $\mathbf y_s \in Y^n$ by minimizing the following objective:
%
\begin{equation}
	L(X_s, \mathbf y_s) = l(\mathbf y, K_{X X_{s}}(K_{X_{s}X_{s}} + \lambda I)^{-1} \mathbf y_s),
	%\label{eq:kip_loss}
\end{equation}
%
where $l$ is the loss function for classification, $K_{X X_s} \in \mathbb R^{N \times n}$ is the NTK matrix between $X$ and $X_s$, $K_{X_s X_s} \in \mathbb R^{n \times n}$ is the NTK matrix of $X_s$ with itself, and $\lambda > 0$ is a regularization hyperparameter.
% We select KIP based on the findings of~\citet{cuiDCBENCHDatasetCondensation2022} where KIP was comparably effective to downstream model-based distillation, while also being the most model-agnostic method that does not rely on the architecture of the downstream model.

\subsection{Testbed Setup: Datasets, Models and Hyperparameter Optimization}
\label{sec:datasets_and_models}
We test each pipeline with 23 open-source tabular datasets, accessed through OpenML~\cite{OpenML2013}, all of which have more than 10,000 rows and 10 features. 
\todo{Better motivate dataset choice: show random vs full data perf on all datasets/estimators

Maybe drop datasets with negative regret for RND}
Each dataset is split to a train, validation and test set with a split of 70\%, 15\%, and 15\%, respectively. The train set is then used to train the autoencoder and later transformed into a distilled dataset in the respective pipelines. We produce distilled datasets with $n/L \in [10, 100]$ labels per class in each pipeline.
\todo{Add note on what kind of compression rates these induce}

The autoencoders are implemented with a latent dimension of size $16$ for every dataset to allow for a fair comparison of the distillation methods across by projecting each dataset to the same space.
We consider five downstream classifiers: XGBoost, K-Nearest Neighbors, Logistic Regression and Naive Bayes as our \textit{shallow} classifiers and MLP, FT-Transformer~\cite{gorishniyRevisitingDeepLearning2021}, Resnet~\cite{gorishniyRevisitingDeepLearning2021} as our \textit{deep} classifier.
Due to time and resource constraints, we train ResNet and FT-Transformer for 5 datasets.
Further discussion on these classifiers can be found in~\cref{apdx:subsec:resnet_ft}.
All of our experiments were conducted on internal HPC clusters equipped with V100 GPUs and x86 CPUs.

% \subsection{Autoencoder Hyperparatemer Optimization}
{\bf Autoencoder Hyperparameter (HP) Optimization. }The HPs considered for the encoder modules of the autoencoders can be found in~\Cref{apdx:tab:hpo:enc:ffn,apdx:tab:hpo:enc:gnn,apdx:tab:hpo:enc:tf}.
% \todo{dont we need to also add/point to the transformer encoder HPs}
\Cref{apdx:tab:hpo:enc:dec} shows the HPs considered for the decoder module, as the architecture is shared for both types of encoders.
The HPs for the classifier head used in the supervised fine-tuning process can be found in~\Cref{apdx:tab:hpo:enc:clf}.

% \subsubsection{Parameter size of autoencoders}

% \subsection{Evaluation Metrics}
%
% The autoencoders are evaluated by their reconstruction accuracy.
% Since all features of the dataset are binarized, we used a normalized sum of the cross-entropy loss to train and evaluate the autoencoders.
%
% We used the balanced accuracy score as the target metric for our downstream classifiers.
% In order to map the difference between a specific pipeline and using the full training data, we also used the \textit{regret} score .
% The regret score is calculated as the following: $(A_{full} - A_{target}) / A_{full}$, where $A_{full}$ is the score of the classifier trained with full data and $A_{target}$ is the score trained with the target distilled data.
%
% In addition, we examine the ranking of the classifiers' performances to compare different components of the distillation pipeline. This is done by ranking the classifier performance trained on pipelines that differ in just one component, where the best performing pipeline was assigned the rank 0. This ranking mechanism allows us to understand how each component contributes to the performance of the downstream classifier under otherwise equal settings.

% \subsubsection{Reconstruction Accuracy}
% We used a modified version of the reconstruction loss function from \Cref{eq:enc:recon_loss} to evaluate the performance of the autoencoders in a metric bound between $[0,1]$.
% The reconstruction accuracy for a row $x$ with n features, with data homogenizer $P$, encoder $\phi$, decoder $\psi$ and group-wise softmax operator $\sigma$ can be expressed as the following dot product:
%
% \begin{equation}
% 	A_{recon} = \frac{1}{n} (P(x) \cdot \sigma(\psi(\phi(P(x))))))
% \end{equation}

% \subsubsection{Classification Accuracy}
% We used balanced accuracy as our target metric to account for the label imbalance of many datasets.
% The balanced accuracy score is defined as follows, using true positive ($TP$), true negative ($TN$), false positive ($FP$), and false negative ($FN$):
% We used this metric to evaluate both the autoencoder classification and the downstream classifiers' performance.

% \begin{equation}
% 	A_{clf} = \frac{1}{2} (\frac{TP}{TP + FN} + \frac{TN}{TN + FP})
% 	\label{eq:balanced_acc}
% \end{equation}

\subsection{Metrics}
{\bf Relative Regret Score.} \label{metrics:regret_score}
We use the balanced accuracy score as the target metric for our downstream classifiers.
In order to map the difference between a specific pipeline and using the full training data, we use what we refer to as the \textit{relative regret} score,
$(A_{F} - A) / (A_{F} - A_{RND@10})$,
where $A_{F}$ is the score of the classifier trained with full data, $A_{RND@10}$ is the score of the classifier trained on 10 randomly sample points, and $A$ is the score trained with the target distilled data.
This metrics maps the performance difference between the current pipeline and 10 randomly sampled points with respect to training on the full data, where \textit{lower is better}.

{\bf Ranking.}
We use the aggregate ranking of different pipelines to compare the efficacy of individual components. For example, if ablating the performance of distillation methods, we group the pipelines that use otherwise equal components -- i.e. same autoencoder, classifier and distillation size -- and aggregate the distillation methods' ranks across all groups.

% and rank their performances based \textit{only} on the distillation methods. The best performer is assigned rank 0.
% \todo{instead of ``rank their performances based \textit{only} on the distillation methods'' I think we want to say ``we use these to rank distillation methods in a single pipeline configuration, and aggregate these ranks across all available pipeline configurations.''}

% More elaborately, with a dataset $S$,  for encoder $E \in \{ \text{FFN}, \text{GNN} \}$, with or without FT (that $F \in \{0, 1\}$), distillation method $DM \in \{ \text{RS}, \text{KM}, \text{AG}, \text{KIP} \} $ with distillation size $n/L \in \{10, 50, 100\}$, output space choice $O \in \{\text{Encoded}, \text{Decoded}\}$ and downstream classifer $M \in \{ \text{NB}, \text{KNN}, \text{LR}, \text{MLP}, \text{XGB} \}$, we can write a pipeline as follows:
% $$
% 	S \to E \oplus F \to DM \oplus n/L \to O \to M.
% $$

% In order to ablate the effect of the distillation method choice, we do the following: For a fixed $M$ (say XGB) and fixed $n/L$ (say $=10$), and over all combinations of $(S, E, F, O)$, we rank the following between $[0,1,2,3]$:
% \begin{itemize}
% 	\item $S \to E \oplus F \to \text{RS} \oplus n/L \to O \to M$,
% 	\item $S \to E \oplus F \to \text{KM} \oplus n/L \to O \to M$,
% 	\item $S \to E \oplus F \to \text{AG} \oplus n/L \to O \to M$,
% 	\item $S \to E \oplus F \to \text{KIP} \oplus n/L \to O \to M$.
% \end{itemize}

% This process results in multiple sets of rankings of the distillation methods with different components, which we then plot the distribution of, where the best performance is ranked at 0.
% Thus, each boxplot in each subfigure of \Cref{fig:os_rank_dist} corresponds to the list of ranks for the distillation method obtained from the above procedure.
% We apply this process to ablate the effect of any one choice in the pipeline.

% \todo[inline]{Discuss ranking procedure in detail with examples}
%\todo[inline]{check if this detailed ranking procedure makes sense to add}
% \todo[inline]{inwon: Just changed $D$ to $DM$ since we use $D$ for binarized data dimension
% \\pr: good catch! thanks for fixing.}



==> related_work.tex <==
\section{Related Work}

{\tiny \begin{itemize}
\item Highlight how most methods are model-specific; relies on model differentiability (bilevel formulation)
\item Discuss DC bench results
\item Also position properly against coreset selection and synthetic tabular data generation
\item say k-means etc are coreset selection schemes
\item for generative models for synthetic data generation, the goal to generate ``realistic samples''. Quoting from \citet{yu2023dataset}, {\em `` generative models try to synthesize realistic images, while DD cares about generating informative images that can boost training efficiency and save storage costs.''}
\end{itemize}}


{\bf Dataset Distillation.}
Unlike model or knowledge distillation~\cite{deng2020model,fakoor2020fast,gou2021knowledge,yang2023effective,zhao2021dataset} which aim to produce a smaller model from a larger model, dataset distillation aims to produce a smaller dataset that that is \textit{model-agnostic} and has uses other than producing an ML model Due to the prevalence of NN models in computer vision, past works in this field focus on an NN-based method of distilling image datasets.
\citet{wangDatasetDistillation2020} introduced the concept of dataset distillation in image datasets by learning a new dataset that minimizes the target model's performance difference between the original dataset and the distilled dataset.
The following literature then considered methods that leverage the parameter gradient of the target model instead of the parameters~\cite{cazenavetteDatasetDistillationMatching2022b,nguyenDatasetMetaLearningKernel2021,zhao2021dataset}.
~\citet{zhao2021dataset} propose matching the target model's gradient produced from the original and distilled dataset at each training iteration.
~\citet{nguyenDatasetMetaLearningKernel2021} introduce a kernel-inducing points (KIP) algorithm, which uses kernel ridge regression (KRR) with the neural tangent kernel (NTK)~\cite{jacotNeuralTangentKernel2018} of a wide neural network to approximate its training and train a synthetic (distilled) dataset.
Finally,~\citet{cui2022dc} perform a survey and experiment to benchmark six different data distillation methods, reporting that trajectory matching~\cite{cazenavetteDatasetDistillationMatching2022b} performs the best, with KIP~\cite{nguyenDatasetMetaLearningKernel2021} following the second.
The authors also consider \textit{k}-means algorithm as one of the baseline methods and note that it performs better than many other model-based distillation methods considered in the study, which is confirmed in our findings.
In this work, we consider gradient matching (GM) and KIP and in this work due to the fact that~\citet{cazenavetteDatasetDistillationMatching2022b} considers a heavily NN-reliant and \textit{model-centric} method while GM algorithm is not as heavily reliant on the target model and KIP treats the NN as a kernel machine.

Coreset selection, the task of finding a \textit{representative subset} given a dataset, is another line of work closely related data distllation.
Clustering methods have been closely studied~\cite{ClusteringMillionsFaces,chaiEfficientCoresetSelection2023,davidsonCorsetEnablingDifferential2014,har-peledSmallerCoresetsKMedian,mirzasoleimanCoresetsDataefficientTraining2020}.
In particular, we focus on two types of clustering algorithms commonly found in the literature, i.e. $k$-means~\cite{chaiEfficientCoresetSelection2023,har-peledSmallerCoresetsKMedian,mirzasoleimanCoresetsDataefficientTraining2020} and agglomerative clustering~\cite{ClusteringMillionsFaces,davidsonCorsetEnablingDifferential2014}.

{\bf Tabular Data.} 
Feature reduction is another closely related area of dataset distillation which has been explored in terms of tabular datasets~\cite{basgall2021fdr2,makridis2020predictive,piramuthu2005feature,sammany2007dimensionality} unlike dataset distillation.
However, feature reduction aims to reduce the number of features in a dataset, rather than the number of samples.
This work focuses on reducing the number of samples in a dataset, which results in a smaller dataset than feature reduction, as datasets tend to have more samples than features.

\citet{medvedevNewPropertiesData2021a} discuss the properties of tabular data distillation by exploring the method proposed by~\citet{wangDatasetDistillation2020}.
However, it only considers a synthetic dataset with a NN model, which does not address the full scope of the problem.
\citet{wuOpenWorldFeatureExtrapolation2021} proposes a graph neural network (GNN)-based architecture to handle tabular datasets by leveraging features' interactions.
Our previous work also proposed and described the preliminary results of tabular data distillation~\cite{kang2024effective}, which we expand upon with full details and additional result analysis in this work.
We use this architecture as one of the autoencoders considered in this work.


==> tables/iclr-rebuttal/rq2-compare-distill-method-n100.tex <==
\begin{tabular}{llcccccc}
\toprule
Distill Method & Encoder & \multicolumn{6}{c}{Regret} \\
 &  & Min & Q1 & Mean & Median & Q3 & Max \\
\midrule
Random Sample & N/A & 0.0605 & 0.2865 & 0.4779 & 0.4847 & 0.6056 & 0.9970 \\
\midrule
KM &  TF & 0.0317 & 0.2424 & 0.4108 & 0.3957 & 0.5026 & 0.8505 \\
\midrule
AG &  TF & 0.0398 & 0.1986 & 0.3802 & 0.3858 & 0.5509 & 0.7658 \\
\midrule
KIP &  TF & 0.0582 & 0.4524 & 0.7051 & 0.6832 & 0.9303 & 1.4403 \\
\midrule
GM &  TF & 0.1301 & 0.4051 & 0.6819 & 0.5577 & 1.0004 & 1.4634 \\
\midrule
FG &  TF & 0.4454 & 1.1062 & 2.5191 & 1.5241 & 2.4758 & 17.0818 \\
\midrule
GN &  TF & 0.9291 & 1.0997 & 1.5733 & 1.3601 & 1.8184 & 3.8737 \\
\midrule
GL &  TF & 0.8963 & 1.0491 & 1.5831 & 1.2018 & 1.6676 & 6.0045 \\
\midrule
GC &  TF & -0.0454 & 0.6036 & 0.9720 & 0.8454 & 1.1346 & 2.9342 \\
\midrule
MTT &  TF & 0.1387 & 0.4051 & 0.6882 & 0.5960 & 1.0040 & 1.4715 \\
DATM &  TF & 0.1387 & 0.4051 & 0.6882 & 0.5960 & 1.0040 & 1.4715 \\
\bottomrule
\end{tabular}


==> tables/iclr-rebuttal/rq2-compare-distill-method-n50.tex <==
\begin{tabular}{llcccccc}
\toprule
Distill Method & Encoder & \multicolumn{6}{c}{Regret} \\
 &  & Min & Q1 & Mean & Median & Q3 & Max \\
\midrule
Random Sample & N/A & 0.2523 & 0.4002 & 0.6016 & 0.5334 & 0.7150 & 1.1035 \\
\midrule
KM &  TF & 0.0982 & 0.3040 & 0.4786 & 0.4795 & 0.6358 & 0.8551 \\
\midrule
AG &  TF & 0.0000 & 0.3037 & 0.4340 & 0.4842 & 0.5177 & 0.8312 \\
\midrule
KIP &  TF & 0.1580 & 0.5060 & 0.7571 & 0.7209 & 0.9603 & 1.4614 \\
\midrule
GM &  TF & 0.1711 & 0.4695 & 0.7374 & 0.6591 & 0.9094 & 1.4808 \\
\midrule
FG &  TF & 0.5149 & 1.1094 & 2.4900 & 1.4958 & 2.2200 & 17.0558 \\
\midrule
GN &  TF & 0.8521 & 1.1584 & 1.7059 & 1.3988 & 1.9306 & 5.4406 \\
\midrule
GL &  TF & 0.7609 & 1.0677 & 1.8477 & 1.2449 & 1.7963 & 10.2800 \\
\midrule
GC &  TF & 0.2468 & 0.7302 & 1.1657 & 0.9251 & 1.4984 & 4.5673 \\
\midrule
MTT &  TF & 0.2282 & 0.4787 & 0.7679 & 0.6670 & 0.9119 & 1.6127 \\
DATM &  TF & 0.2282 & 0.4787 & 0.7679 & 0.6670 & 0.9119 & 1.6127 \\
\bottomrule
\end{tabular}


==> tables/rq1_1-compare-col-emb-n100.tex <==
\begin{tabular}{lcccc}
\toprule
Col. Emb. & KM & AG & GM & KIP \\
\midrule
Binary & $_{-0.1717}$ 0.1409 $_{0.4304}$ & $_{-0.1316}$ 0.1452 $_{0.4614}$ & $_{0.1742}$ 0.3281 $_{0.4906}$ & $_{0.1428}$ 0.4270 $_{0.8298}$ \\
Scaled & $_{0.2558}$ 0.3363 $_{0.5173}$ & $_{0.1814}$ 0.3133 $_{0.5597}$ & $_{0.9228}$ 1.3435 $_{1.8914}$ & $_{0.9171}$ 1.4782 $_{1.8513}$ \\
PLE & $_{-0.5257}$ 0.2190 $_{0.3771}$ & $_{-0.5015}$ 0.2646 $_{0.4617}$ & $_{-0.2416}$ 0.0799 $_{0.5522}$ & $_{-0.0786}$ 0.2064 $_{0.6113}$ \\
\bottomrule
\end{tabular}


==> tables/rq1_1-compare-col-emb-n50.tex <==
\begin{tabular}{lcccc}
\toprule
Col. Emb. & KM & AG & GM & KIP \\
\midrule
Binary & $_{0.0597}$ 0.3300 $_{0.5557}$ & $_{-0.1606}$ 0.1905 $_{0.4566}$ & $_{0.2514}$ 0.5563 $_{0.8362}$ & $_{0.3641}$ 0.6312 $_{0.9548}$ \\
Scaled & $_{0.3863}$ 0.4838 $_{0.6647}$ & $_{0.3618}$ 0.5136 $_{0.8002}$ & $_{0.9542}$ 1.3818 $_{1.8841}$ & $_{0.9278}$ 1.3799 $_{1.7580}$ \\
PLE & $_{-0.4979}$ 0.2953 $_{0.4920}$ & $_{-0.2603}$ 0.2758 $_{0.5162}$ & $_{-0.2287}$ 0.0859 $_{0.6177}$ & $_{-0.0829}$ 0.1782 $_{0.7064}$ \\
\bottomrule
\end{tabular}


==> tables/rq2-compare-distill-method-n100.tex <==
\begin{tabular}{llcccccc}
\toprule
Distill Method & Encoder & \multicolumn{6}{c}{Regret} \\
 &  & Min & Q1 & Mean & Median & Q3 & Max \\
\midrule
Random Sample & N/A & -11.0609 & 0.2589 & 0.1842 & 0.3753 & 0.5818 & 5.4937 \\
\midrule
KM &  TF & -25.4981 & 0.0000 & -0.4711 & 0.2177 & 0.4305 & 1.1158 \\
KM &  FFN & -21.6299 & 0.0051 & -0.3587 & 0.1938 & 0.4449 & 0.9201 \\
KM &  GNN & -16.7865 & 0.0000 & -0.4087 & 0.1826 & 0.3972 & 0.8376 \\
\midrule
AG &  TF & -19.8902 & 0.0000 & -0.3581 & 0.2018 & 0.4539 & 1.1052 \\
AG &  FFN & -16.4911 & 0.0000 & -0.3752 & 0.2293 & 0.4229 & 0.8694 \\
AG &  GNN & -13.1186 & 0.0063 & -0.2379 & 0.2019 & 0.4195 & 1.0130 \\
\midrule
KIP &  TF & -12.6254 & 0.1684 & 0.3305 & 0.4396 & 0.8083 & 10.0877 \\
KIP &  FFN & -12.1272 & 0.1844 & 0.7260 & 0.7064 & 1.0802 & 14.1880 \\
KIP &  GNN & -8.1696 & 0.2004 & 0.3763 & 0.4464 & 0.8031 & 6.1959 \\
\midrule
GM &  TF & -11.6940 & 0.1250 & 0.0974 & 0.3387 & 0.7093 & 1.4869 \\
GM &  FFN & -12.2809 & 0.1693 & 0.4587 & 0.5141 & 0.8467 & 11.7744 \\
GM &  GNN & -10.8773 & 0.1191 & 0.0664 & 0.3387 & 0.6077 & 1.4489 \\
\bottomrule
\end{tabular}


==> tables/rq2-compare-distill-method-n50.tex <==
\begin{tabular}{llcccccc}
\toprule
Distill Method & Encoder & \multicolumn{6}{c}{Regret} \\
 &  & Min & Q1 & Mean & Median & Q3 & Max \\
\midrule
Random Sample & N/A & -5.6993 & 0.4065 & 0.5401 & 0.5475 & 0.7218 & 6.2160 \\
\midrule
KM &  TF & -22.5086 & 0.0042 & -0.3555 & 0.2663 & 0.4922 & 1.1067 \\
KM &  FFN & -20.8030 & 0.0707 & -0.2245 & 0.2981 & 0.5525 & 0.9423 \\
KM &  GNN & -13.7989 & 0.0122 & -0.2441 & 0.2979 & 0.4704 & 0.9231 \\
\midrule
AG &  TF & -22.4617 & 0.0000 & -0.3004 & 0.2311 & 0.4943 & 1.1722 \\
AG &  FFN & -11.4505 & 0.0382 & -0.1309 & 0.3235 & 0.5732 & 0.9720 \\
AG &  GNN & -13.0925 & 0.0841 & -0.1274 & 0.2800 & 0.4612 & 0.9939 \\
\midrule
KIP &  TF & -10.5707 & 0.2157 & 0.4000 & 0.5040 & 0.8791 & 5.7594 \\
KIP &  FFN & -8.5167 & 0.2995 & 0.9689 & 0.8313 & 1.1789 & 16.2155 \\
KIP &  GNN & -6.1155 & 0.3059 & 0.6189 & 0.6154 & 0.8728 & 10.5023 \\
\midrule
GM &  TF & -8.3684 & 0.1744 & 0.3215 & 0.4661 & 0.8055 & 4.2983 \\
GM &  FFN & -10.5816 & 0.3358 & 0.7755 & 0.7491 & 1.0110 & 12.4418 \\
GM &  GNN & -7.4118 & 0.2531 & 0.3879 & 0.4981 & 0.8229 & 1.4901 \\
\bottomrule
\end{tabular}

